ODIN: Overcoming Dynamic Interference in iNference pipelines

As an increasing number of businesses becomes powered by machine-learning, inference becomes a core operation, with a growing trend to be offered as a service. In this context, the inference task must meet certain service-level objectives (SLOs), such as high throughput and low latency. However, these targets can be compromised by interference caused by long- or short-lived co-located tasks. Prior works focus on the generic problem of co-scheduling to mitigate the effect of interference on the performance-critical task. In this work, we focus on inference pipelines and propose ODIN, a technique to mitigate the effect of interference on the performance of the inference task, based on the online scheduling of the pipeline stages. Our technique detects interference online and automatically re-balances the pipeline stages to mitigate the performance degradation of the inference task. We demonstrate that ODIN successfully mitigates the effect of interference, sustaining the latency and throughput of CNN inference, and outperforms the least-loaded scheduling (LLS), a common technique for interference mitigation. Additionally, it is effective in maintaining service-level objectives for inference, and it is scalable to large network models executing on multiple processing elements.

==> comments.tex <==
\newboolean{showcomments}
\setboolean{showcomments}{true}
\makeatletter
\newcommand{\mynote}[3]{%
  \ifthenelse{\boolean{showcomments}}{%
   \fbox{\bfseries\sffamily\scriptsize#1}%
   {\small$\blacktriangleright$\textsf{\emph{\color{#3}{#2}}}$\blacktriangleleft$}}%
  {%
   % these two lines ensure that there is no blank space inserted 
   \@bsphack
   \@esphack
  }%
}
\makeatother

% One command per author:
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\newcommand{\jc}[1]{\mynote{Jeronimo}{#1}{asparagus}}
\definecolor{something}{rgb}{0.2, 0.2, 0.6}
\newcommand{\pns}[1]{\mynote{Pirah}{#1}{something}}
\definecolor{something1}{rgb}{0.6, 0.2, 0.2}
\newcommand{\miquel}[1]{\mynote{Miquel}{#1}{something1}}
\definecolor{something2}{rgb}{0.6, 0.6, 0.2}
\newcommand{\ma}[1]{\mynote{Mustafa}{#1}{something2}}
\definecolor{something3}{rgb}{0.6, 0.2, 0.6}
\newcommand{\nr}[1]{\mynote{Norman}{#1}{something3}}

==> old_references.tex <==
@inproceedings{yadwadkar2019case,
  title={A case for managed and model-less inference serving},
  author={Yadwadkar, Neeraja J and Romero, Francisco and Li, Qian and Kozyrakis, Christos},
  booktitle={Proceedings of the Workshop on Hot Topics in Operating Systems},
  pages={184--191},
  year={2019}
}
@article{delimitrou2013paragon,
  title={Paragon: QoS-aware scheduling for heterogeneous datacenters},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={48},
  number={4},
  pages={77--88},
  year={2013},
  publisher={ACM New York, NY, USA}
}
@article{devi2016load,
  title={Load balancing in cloud computing environment using improved weighted round robin algorithm for nonpreemptive dependent tasks},
  author={Devi, D Chitra and Uthariaraj, V Rhymend},
  journal={The scientific world journal},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}
@inproceedings{shaw2014survey,
  title={A survey on scheduling and load balancing techniques in cloud computing environment},
  author={Shaw, Subhadra Bose and Singh, AK},
  booktitle={2014 international conference on computer and communication technology (ICCCT)},
  pages={87--95},
  year={2014},
  organization={IEEE}
}
@article{delimitrou2014quasar,
  title={Quasar: Resource-efficient and qos-aware cluster management},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={49},
  number={4},
  pages={127--144},
  year={2014},
  publisher={ACM New York, NY, USA}
}
@inproceedings{romero2018mage,
  title={Mage: Online and interference-aware scheduling for multi-scale heterogeneous systems},
  author={Romero, Francisco and Delimitrou, Christina},
  booktitle={Proceedings of the 27th International Conference on Parallel Architectures and Compilation Techniques},
  pages={1--13},
  year={2018}
}
@inproceedings{mendoza2021interference,
  title={Interference-aware scheduling for inference serving},
  author={Mendoza, Daniel and Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={Proceedings of the 1st Workshop on Machine Learning and Systems},
  pages={80--88},
  year={2021}
}
@inproceedings{ke2022hercules,
  title={Hercules: Heterogeneity-Aware Inference Serving for At-Scale Personalized Recommendation},
  author={Ke, Liu and Gupta, Udit and Hempsteadis, Mark and Wu, Carole-Jean and Lee, Hsien-Hsin S and Zhang, Xuan},
  booktitle={2022 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={141--144},
  year={2022},
  organization={IEEE}
}
@inproceedings{delimitrou2013ibench,
  title={ibench: Quantifying interference for datacenter applications},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  booktitle={2013 IEEE international symposium on workload characterization (IISWC)},
  pages={23--33},
  year={2013},
  organization={IEEE}
}
@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang, Yanping and Cheng, Youlong and Bapna, Ankur and Firat, Orhan and Chen, Dehao and Chen, Mia and Lee, HyoukJoong and Ngiam, Jiquan and Le, Quoc V and Wu, Yonghui and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@inproceedings{narayanan2019pipedream,
  title={PipeDream: generalized pipeline parallelism for DNN training},
  author={Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R and Ganger, Gregory R and Gibbons, Phillip B and Zaharia, Matei},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={1--15},
  year={2019}
}
@article{soomro2022shisha,
  title={Shisha: Online scheduling of CNN pipelines on heterogeneous architectures},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  journal={arXiv preprint arXiv:2202.11575},
  year={2022}
}
@inproceedings{alves2020interference,
  title={An Interference-Aware Strategy for Co-locating High Performance Computing Applications in Clouds},
  author={Alves, Maicon Melo and Teylo, Luan and Frota, Yuri and Drummond, L{\'u}cia Maria de A},
  booktitle={Symposium on High Performance Computing Systems},
  pages={3--20},
  year={2020},
  organization={Springer}
}
@inproceedings{patel2020clite,
  title={Clite: Efficient and qos-aware co-location of multiple latency-critical jobs for warehouse scale computers},
  author={Patel, Tirthak and Tiwari, Devesh},
  booktitle={2020 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={193--206},
  year={2020},
  organization={IEEE}
}
@inproceedings{alipourfard2017cherrypick,
  title={$\{$CherryPick$\}$: Adaptively Unearthing the Best Cloud Configurations for Big Data Analytics},
  author={Alipourfard, Omid and Liu, Hongqiang Harry and Chen, Jianshu and Venkataraman, Shivaram and Yu, Minlan and Zhang, Ming},
  booktitle={14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
  pages={469--482},
  year={2017}
}
@ARTICLE{9747991,
  author={Rotem, Efraim and Yoaz, Adi and Rappoport, Lihu and Robinson, Stephen J. and Mandelblat, Julius Yuli and Gihon, Arik and Weissmann, Eliezer and Chabukswar, Rajshree and Basin, Vadim and Fenger, Russell and Gupta, Monica and Yasin, Ahmad},
  journal={IEEE Micro}, 
  title={Intel Alder Lake CPU Architectures}, 
  year={2022},
  volume={42},
  number={3},
  pages={13-19},
  doi={10.1109/MM.2022.3164338}}
@article{chang2022pipebert,
  title={PipeBERT: High-throughput BERT Inference for ARM Big. LITTLE Multi-core Processors},
  author={Chang, Hung-Yang and Mozafari, Seyyed Hasan and Chen, Cheng and Clark, James J and Meyer, Brett H and Gross, Warren J},
  journal={Journal of Signal Processing Systems},
  pages={1--18},
  year={2022},
  publisher={Springer}
}
@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang, Yanping and Cheng, Youlong and Bapna, Ankur and Firat, Orhan and Chen, Dehao and Chen, Mia and Lee, HyoukJoong and Ngiam, Jiquan and Le, Quoc V and Wu, Yonghui and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@inproceedings{romero2021infaas,
  title={INFaaS: Automated Model-less Inference Serving.},
  author={Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={USENIX Annual Technical Conference},
  pages={397--411},
  year={2021}
}

@inproceedings{lee2018pretzel,
  title={PRETZEL: Opening the Black Box of Machine Learning Prediction Serving Systems.},
  author={Lee, Yunseong and Scolari, Alberto and Chun, Byung-Gon and Santambrogio, Marco Domenico and Weimer, Markus and Interlandi, Matteo},
  booktitle={OSDI},
  volume={18},
  pages={611--626},
  year={2018}
}


@inproceedings{zhang2019mark,
  title={MArk: Exploiting Cloud Services for Cost-Effective, SLO-Aware Machine Learning Inference Serving.},
  author={Zhang, Chengliang and Yu, Minchen and Wang, Wei and Yan, Feng},
  booktitle={USENIX Annual Technical Conference},
  pages={1049--1062},
  year={2019}
}

@inproceedings{mendoza2021interference,
  title={Interference-aware scheduling for inference serving},
  author={Mendoza, Daniel and Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={Proceedings of the 1st Workshop on Machine Learning and Systems},
  pages={80--88},
  year={2021}
}

@inproceedings{yeung2020horus,
  title={Horus: An interference-aware resource manager for deep learning systems},
  author={Yeung, Gingfung and Borowiec, Damian and Yang, Renyu and Friday, Adrian and Harper, Richard and Garraghan, Peter},
  booktitle={Algorithms and Architectures for Parallel Processing: 20th International Conference, ICA3PP 2020, New York City, NY, USA, October 2--4, 2020, Proceedings, Part II 20},
  pages={492--508},
  year={2020},
  organization={Springer}
}

@article{delimitrou2014quasar,
  title={Quasar: Resource-efficient and QoS-aware cluster management},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={49},
  number={4},
  pages={127--144},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@article{delimitrou2013paragon,
  title={Paragon: QoS-aware scheduling for heterogeneous datacenters},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={48},
  number={4},
  pages={77--88},
  year={2013},
  publisher={ACM New York, NY, USA}
}

@inproceedings{chen2017prophet,
  title={Prophet: Precise qos prediction on non-preemptive accelerators to improve utilization in warehouse-scale computers},
  author={Chen, Quan and Yang, Hailong and Guo, Minyi and Kannan, Ram Srivatsa and Mars, Jason and Tang, Lingjia},
  booktitle={Proceedings of the Twenty-Second International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={17--32},
  year={2017}
}

@article{chen2016baymax,
  title={Baymax: Qos awareness and increased utilization for non-preemptive accelerators in warehouse scale computers},
  author={Chen, Quan and Yang, Hailong and Mars, Jason and Tang, Lingjia},
  journal={ACM SIGPLAN Notices},
  volume={51},
  number={4},
  pages={681--696},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{lo2015heracles,
  title={Heracles: Improving resource efficiency at scale},
  author={Lo, David and Cheng, Liqun and Govindaraju, Rama and Ranganathan, Parthasarathy and Kozyrakis, Christos},
  booktitle={Proceedings of the 42nd Annual International Symposium on Computer Architecture},
  pages={450--462},
  year={2015}
}

@inproceedings{crankshaw2017clipper,
  title={Clipper: A Low-Latency Online Prediction Serving System.},
  author={Crankshaw, Daniel and Wang, Xin and Zhou, Giulio and Franklin, Michael J and Gonzalez, Joseph E and Stoica, Ion},
  booktitle={NSDI},
  volume={17},
  pages={613--627},
  year={2017}
}

@article{olston2017tensorflow,
  title={Tensorflow-serving: Flexible, high-performance ml serving},
  author={Olston, Christopher and Fiedel, Noah and Gorovoy, Kiril and Harmsen, Jeremiah and Lao, Li and Li, Fangwei and Rajashekhar, Vinu and Ramesh, Sukriti and Soyke, Jordan},
  journal={arXiv preprint arXiv:1712.06139},
  year={2017}
}

@inproceedings{liberty2020elastic,
  title={Elastic machine learning algorithms in amazon sagemaker},
  author={Liberty, Edo and Karnin, Zohar and Xiang, Bing and Rouesnel, Laurence and Coskun, Baris and Nallapati, Ramesh and Delgado, Julio and Sadoughi, Amir and Astashonok, Yury and Das, Piali and others},
  booktitle={Proceedings of the 2020 ACM SIGMOD International Conference on Management of Data},
  pages={731--737},
  year={2020}
}

@inproceedings{romero2021infaas,
  title={INFaaS: Automated Model-less Inference Serving.},
  author={Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={USENIX Annual Technical Conference},
  pages={397--411},
  year={2021}
}

@inproceedings{lemay2020perseus,
  title={Perseus: Characterizing performance and cost of multi-tenant serving for cnn models},
  author={LeMay, Matthew and Li, Shijian and Guo, Tian},
  booktitle={2020 IEEE International Conference on Cloud Engineering (IC2E)},
  pages={66--72},
  year={2020},
  organization={IEEE}
}

@inproceedings{ke2022hercules,
  title={Hercules: Heterogeneity-aware inference serving for at-scale personalized recommendation},
  author={Ke, Liu and Gupta, Udit and Hempsteadis, Mark and Wu, Carole-Jean and Lee, Hsien-Hsin S and Zhang, Xuan},
  booktitle={2022 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={141--144},
  year={2022},
  organization={IEEE}
}

@inproceedings{narayanan2019pipedream,
  title={PipeDream: Generalized pipeline parallelism for DNN training},
  author={Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R and Ganger, Gregory R and Gibbons, Phillip B and Zaharia, Matei},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={1--15},
  year={2019}
}

@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang, Yanping and Cheng, Youlong and Bapna, Ankur and Firat, Orhan and Chen, Dehao and Chen, Mia and Lee, HyoukJoong and Ngiam, Jiquan and Le, Quoc V and Wu, Yonghui and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{fan2021dapple,
  title={DAPPLE: A pipelined data parallel approach for training large models},
  author={Fan, Shiqing and Rong, Yi and Meng, Chen and Cao, Zongyan and Wang, Siyu and Zheng, Zhen and Wu, Chuan and Long, Guoping and Yang, Jun and Xia, Lixue and others},
  booktitle={Proceedings of the 26th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
  pages={431--445},
  year={2021}
}

@inproceedings{li2021chimera,
  title={Chimera: efficiently training large-scale neural networks with bidirectional pipelines},
  author={Li, Shigang and Hoefler, Torsten},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}

@article{wang2019high,
  title={High-throughput cnn inference on embedded arm big. little multicore processors},
  author={Wang, Siqi and Ananthanarayanan, Gayathri and Zeng, Yifan and Goel, Neeraj and Pathania, Anuj and Mitra, Tulika},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={10},
  pages={2254--2267},
  year={2019},
  publisher={IEEE}
}

@article{kang2020scheduling,
  title={Scheduling of deep learning applications onto heterogeneous processors in an embedded device},
  author={Kang, Duseok and Oh, Jinwoo and Choi, Jongwoo and Yi, Youngmin and Ha, Soonhoi},
  journal={IEEE Access},
  volume={8},
  pages={43980--43991},
  year={2020},
  publisher={IEEE}
}

@article{jeong2021deep,
  title={Deep learning inference parallelization on heterogeneous processors with tensorrt},
  author={Jeong, EunJin and Kim, Jangryul and Tan, Samnieng and Lee, Jaeseong and Ha, Soonhoi},
  journal={IEEE Embedded Systems Letters},
  volume={14},
  number={1},
  pages={15--18},
  year={2021},
  publisher={IEEE}
}

@article{soomro2022shisha,
  title={Shisha: Online scheduling of CNN pipelines on heterogeneous architectures},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Pericas, Miquel},
  journal={arXiv preprint arXiv:2202.11575},
  year={2022}
}

@inproceedings{soomro2021online,
  title={An online guided tuning approach to run cnn pipelines on edge devices},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={Proceedings of the 18th ACM International Conference on Computing Frontiers},
  pages={45--53},
  year={2021}
}

@article{chang2022pipebert,
  title={PipeBERT: High-throughput BERT Inference for ARM Big. LITTLE Multi-core Processors},
  author={Chang, Hung-Yang and Mozafari, Seyyed Hasan and Chen, Cheng and Clark, James J and Meyer, Brett H and Gross, Warren J},
  journal={Journal of Signal Processing Systems},
  pages={1--18},
  year={2022},
  publisher={Springer}
}

@article{ben2019demystifying,
  title={Demystifying parallel and distributed deep learning: An in-depth concurrency analysis},
  author={Ben-Nun, Tal and Hoefler, Torsten},
  journal={ACM Computing Surveys (CSUR)},
  volume={52},
  number={4},
  pages={1--43},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{lee2015fly,
  title={On-the-fly pipeline parallelism},
  author={Lee, I-Ting Angelina and Leiserson, Charles E and Schardl, Tao B and Zhang, Zhunping and Sukha, Jim},
  journal={ACM Transactions on Parallel Computing (TOPC)},
  volume={2},
  number={3},
  pages={1--42},
  year={2015},
  publisher={ACM New York, NY, USA}
}
@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}
@misc{gitlink,   
    title = {cnn-benchmarks},   
    url = {https://github.com/jcjohnson/cnn-benchmarks},   
    author = {Justin Johnson},   
    year = {2017},   
    note = {Accessed on March 2nd, 2023} 
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

==> relatedWork.tex <==
\section{Related Work}
The effects of interference due to co-locating applications have been studied in detail. 
Most of the previous work is inclined towards providing a proactive solution towards interference.
Interference aware serving systems~\cite{ke2022hercules, mendoza2021interference} and interference aware schedulers in clouds~\cite{delimitrou2013paragon, romero2018mage, delimitrou2014quasar} exploit detailed information on the characteristics of co-locating application and platform. Such as the behavior of application is realized either by data driven approaches~\cite{romero2018mage}, given the data of previous runs or by testing the application under the effects of several micro benchmarks to analyze the sensitivity of application towards different interference scenarios~\cite{delimitrou2013paragon, delimitrou2014quasar}.
The problem with most of the approaches is that either they do not provide a solution if the proactive measure goes wrong~\cite{delimitrou2014quasar, soomro2022shisha,mendoza2021interference,alves2020interference}, what actions should be performed to mitigate interference or the solution is either migrating the whole application or assigning more resources~\cite{delimitrou2013paragon, romero2018mage}, which in case of interactive inference models such as recommendation systems[xxx] is not a viable solution. 

Another component of previous solutions is exploring the complex design space that is comprised of various application features and hardware specification in order to optimize the assignment and co-location of applications on computing resources.
Various methods are proposed for exploration such as collaborative filtering~\cite{delimitrou2013paragon, delimitrou2014quasar}, Bayesian optimization~\cite{patel2020clite,alipourfard2017cherrypick} and machine learning based prediction~\cite{romero2018mage, ke2022hercules, mendoza2021interference}. The problem with these approaches is that they do not, or partially support the online adaptation of the application on available computing platforms. 
To the author's knowledge, a fully online interference mitigation strategy towards co-located application is not explored yet.  

==> scratch_references <==
@inproceedings{yadwadkar2019case,
  title={A case for managed and model-less inference serving},
  author={Yadwadkar, Neeraja J and Romero, Francisco and Li, Qian and Kozyrakis, Christos},
  booktitle={Proceedings of the Workshop on Hot Topics in Operating Systems},
  pages={184--191},
  year={2019}
}
@article{delimitrou2013paragon,
  title={Paragon: QoS-aware scheduling for heterogeneous datacenters},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={48},
  number={4},
  pages={77--88},
  year={2013},
  publisher={ACM New York, NY, USA}
}
@article{devi2016load,
  title={Load balancing in cloud computing environment using improved weighted round robin algorithm for nonpreemptive dependent tasks},
  author={Devi, D Chitra and Uthariaraj, V Rhymend},
  journal={The scientific world journal},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}
@inproceedings{shaw2014survey,
  title={A survey on scheduling and load balancing techniques in cloud computing environment},
  author={Shaw, Subhadra Bose and Singh, AK},
  booktitle={ICCCT},
  pages={87--95},
  year={2014},
  organization={IEEE}
}
@inproceedings{romero2018mage,
  title={Mage: Online and interference-aware scheduling for multi-scale heterogeneous systems},
  author={Romero, Francisco and Delimitrou, Christina},
  booktitle={PACT},
  pages={1--13},
  year={2018}
}
@inproceedings{delimitrou2013ibench,
  title={ibench: Quantifying interference for datacenter applications},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  booktitle={IISWC},
  pages={23--33},
  year={2013},
  organization={IEEE}
}
@inproceedings{alves2020interference,
  title={An Interference-Aware Strategy for Co-locating High Performance Computing Applications in Clouds},
  author={Alves, Maicon Melo and Teylo, Luan and Frota, Yuri and Drummond, L{\'u}cia Maria de A},
  booktitle={Symposium on High Performance Computing Systems},
  pages={3--20},
  year={2020},
  organization={Springer}
}
@inproceedings{patel2020clite,
  title={Clite: Efficient and qos-aware co-location of multiple latency-critical jobs for warehouse scale computers},
  author={Patel, Tirthak and Tiwari, Devesh},
  booktitle={HPCA},
  pages={193--206},
  year={2020},
  organization={IEEE}
}
@inproceedings{alipourfard2017cherrypick,
  title={$\{$CherryPick$\}$: Adaptively Unearthing the Best Cloud Configurations for Big Data Analytics},
  author={Alipourfard, Omid and Liu, Hongqiang Harry and Chen, Jianshu and Venkataraman, Shivaram and Yu, Minlan and Zhang, Ming},
  booktitle={14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
  pages={469--482},
  year={2017}
}
@ARTICLE{9747991,
  author={Rotem, Efraim and Yoaz, Adi and Rappoport, Lihu and Robinson, Stephen J. and Mandelblat, Julius Yuli and Gihon, Arik and Weissmann, Eliezer and Chabukswar, Rajshree and Basin, Vadim and Fenger, Russell and Gupta, Monica and Yasin, Ahmad},
  journal={IEEE Micro}, 
  title={Intel Alder Lake CPU Architectures}, 
  year={2022},
  volume={42},
  number={3},
  pages={13-19},
  doi={10.1109/MM.2022.3164338}}

@inproceedings{lee2018pretzel,
  title={PRETZEL: Opening the Black Box of Machine Learning Prediction Serving Systems.},
  author={Lee, Yunseong and Scolari, Alberto and Chun, Byung-Gon and Santambrogio, Marco Domenico and Weimer, Markus and Interlandi, Matteo},
  booktitle={OSDI},
  volume={18},
  pages={611--626},
  year={2018}
}


@inproceedings{zhang2019mark,
  title={MArk: Exploiting Cloud Services for Cost-Effective, SLO-Aware Machine Learning Inference Serving.},
  author={Zhang, Chengliang and Yu, Minchen and Wang, Wei and Yan, Feng},
  booktitle={USENIX Annual Technical Conference},
  pages={1049--1062},
  year={2019}
}

@inproceedings{mendoza2021interference,
  title={Interference-aware scheduling for inference serving},
  author={Mendoza, Daniel and Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={Proceedings of the 1st Workshop on Machine Learning and Systems},
  pages={80--88},
  year={2021}
}

@inproceedings{yeung2020horus,
  title={Horus: An interference-aware resource manager for deep learning systems},
  author={Yeung, Gingfung and Borowiec, Damian and Yang, Renyu and Friday, Adrian and Harper, Richard and Garraghan, Peter},
  booktitle={ICA3PP},
  pages={492--508},
  year={2020},
  organization={Springer}
}

@article{delimitrou2014quasar,
  title={Quasar: Resource-efficient and QoS-aware cluster management},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={49},
  number={4},
  pages={127--144},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{chen2017prophet,
  title={Prophet: Precise qos prediction on non-preemptive accelerators to improve utilization in warehouse-scale computers},
  author={Chen, Quan and Yang, Hailong and Guo, Minyi and Kannan, Ram Srivatsa and Mars, Jason and Tang, Lingjia},
  booktitle={Proceedings of the 22nd ASPLOS'17},
  pages={17--32}
}

@article{chen2016baymax,
  title={Baymax: Qos awareness and increased utilization for non-preemptive accelerators in warehouse scale computers},
  author={Chen, Quan and Yang, Hailong and Mars, Jason and Tang, Lingjia},
  journal={ACM SIGPLAN Notices},
  volume={51},
  number={4},
  pages={681--696},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{lo2015heracles,
  title={Heracles: Improving resource efficiency at scale},
  author={Lo, David and Cheng, Liqun and Govindaraju, Rama and Ranganathan, Parthasarathy and Kozyrakis, Christos},
  booktitle={Proceedings of the 42nd Annual International Symposium on Computer Architecture},
  pages={450--462},
  year={2015}
}

@inproceedings{crankshaw2017clipper,
  title={Clipper: A Low-Latency Online Prediction Serving System.},
  author={Crankshaw, Daniel and Wang, Xin and Zhou, Giulio and Franklin, Michael J and Gonzalez, Joseph E and Stoica, Ion},
  booktitle={NSDI},
  year={2017}
}

@article{olston2017tensorflow,
  title={Tensorflow-serving: Flexible, high-performance ml serving},
  author={Olston, Christopher and Fiedel, Noah and Gorovoy, Kiril and Harmsen, Jeremiah and Lao, Li and Li, Fangwei and Rajashekhar, Vinu and Ramesh, Sukriti and Soyke, Jordan},
  journal={arXiv preprint arXiv:1712.06139},
  year={2017}
}

@inproceedings{liberty2020elastic,
  title={Elastic machine learning algorithms in amazon sagemaker},
  author={Liberty, Edo and Karnin, Zohar and Xiang, Bing and Rouesnel, Laurence and Coskun, Baris and Nallapati, Ramesh and Delgado, Julio and Sadoughi, Amir and Astashonok, Yury and Das, Piali and others},
  booktitle={SIGMOD},
  pages={731--737},
  year={2020}
}

@inproceedings{romero2021infaas,
  title={INFaaS: Automated Model-less Inference Serving.},
  author={Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={USENIX Annual Technical Conference},
  pages={397--411},
  year={2021}
}

@inproceedings{lemay2020perseus,
  title={Perseus: Characterizing performance and cost of multi-tenant serving for cnn models},
  author={LeMay, Matthew and Li, Shijian and Guo, Tian},
  booktitle={IC2E},
  pages={66--72},
  year={2020},
  organization={IEEE}
}

@inproceedings{ke2022hercules,
  title={Hercules: Heterogeneity-aware inference serving for at-scale personalized recommendation},
  author={Ke, Liu and Gupta, Udit and Hempsteadis, Mark and Wu, Carole-Jean and Lee, Hsien-Hsin S and Zhang, Xuan},
  booktitle={HPCA},
  pages={141--144},
  year={2022},
  organization={IEEE}
}

@inproceedings{narayanan2019pipedream,
  title={PipeDream: Generalized pipeline parallelism for DNN training},
  author={Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R and Ganger, Gregory R and Gibbons, Phillip B and Zaharia, Matei},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={1--15},
  year={2019}
}

@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{fan2021dapple,
  title={DAPPLE: A pipelined data parallel approach for training large models},
  author={Fan, Shiqing and Rong, Yi and Meng, Chen and Cao, Zongyan and Wang, Siyu and Zheng, Zhen and Wu, Chuan and Long, Guoping and Yang, Jun and Xia, Lixue and others},
  booktitle={Proceedings of the 26th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
  pages={431--445},
  year={2021}
}

@inproceedings{li2021chimera,
  title={Chimera: efficiently training large-scale neural networks with bidirectional pipelines},
  author={Li, Shigang and Hoefler, Torsten},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}

@article{wang2019high,
  title={High-throughput cnn inference on embedded arm big. little multicore processors},
  author={Wang and others},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={10},
  pages={2254--2267},
  year={2019},
  publisher={IEEE}
}

@article{kang2020scheduling,
  title={Scheduling of deep learning applications onto heterogeneous processors in an embedded device},
  author={Kang, Duseok and Oh, Jinwoo and Choi, Jongwoo and Yi, Youngmin and Ha, Soonhoi},
  journal={IEEE Access},
  volume={8},
  year={2020},
  publisher={IEEE}
}

@article{jeong2021deep,
  title={Deep learning inference parallelization on heterogeneous processors with tensorrt},
  author={Jeong, EunJin and Kim, Jangryul and Tan, Samnieng and Lee, Jaeseong and Ha, Soonhoi},
  journal={IEEE Embedded Systems Letters},
  volume={14},
  number={1},
  pages={15--18},
  year={2021},
  publisher={IEEE}
}
@inproceedings{soomro2022shisha,
  title={Shisha: Online scheduling of CNN pipelines on heterogeneous architectures},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={PPAM 2022}
}

@inproceedings{soomro2021online,
  title={An online guided tuning approach to run cnn pipelines on edge devices},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={CF'21}
}

@article{chang2022pipebert,
  title={PipeBERT: High-throughput BERT Inference for ARM Big. LITTLE Multi-core Processors},
  author={Chang, Hung-Yang and Mozafari, Seyyed Hasan and Chen, Cheng and Clark, James J and Meyer, Brett H and Gross, Warren J},
  journal={Journal of Signal Processing Systems},
  pages={1--18},
  year={2022},
  publisher={Springer}
}

@article{ben2019demystifying,
  title={Demystifying parallel and distributed deep learning: An in-depth concurrency analysis},
  author={Ben-Nun, Tal and Hoefler, Torsten},
  journal={ACM Computing Surveys (CSUR)},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{lee2015fly,
  title={On-the-fly pipeline parallelism},
  author={Lee, I-Ting Angelina and Leiserson, Charles E and Schardl, Tao B and Zhang, Zhunping and Sukha, Jim},
  journal={ACM Transactions on Parallel Computing (TOPC)},
  volume={2},
  number={3},
  pages={1--42},
  year={2015},
  publisher={ACM New York, NY, USA}
}
@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}
@misc{gitlink,   
    title = {cnn-benchmarks},   
    url = {https://github.com/jcjohnson/cnn-benchmarks},   
    author = {Justin Johnson},   
    year = {2017},   
    note = {Accessed on March 2nd, 2023} 
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}




























@inproceedings{yadwadkar2019case,
  title={A case for managed and model-less inference serving},
  author={Yadwadkar and others},
  booktitle={Proceedings of the Workshop on Hot Topics in Operating Systems},
  pages={184--191},
  year={2019}
}
@article{delimitrou2013paragon,
  title={Paragon: QoS-aware scheduling for heterogeneous datacenters},
  author={Delimitrou and others},
  journal={ACM SIGPLAN Notices},
  volume={48},
  number={4},
  pages={77--88},
  year={2013},
  publisher={ACM New York, NY, USA}
}
@article{devi2016load,
  title={Load balancing in cloud computing environment using improved weighted round robin algorithm for nonpreemptive dependent tasks},
  author={Devi and others},
  journal={The scientific world journal},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}
@inproceedings{shaw2014survey,
  title={A survey on scheduling and load balancing techniques in cloud computing environment},
  author={Shaw and others},
  booktitle={ICCCT},
  pages={87--95},
  year={2014},
  organization={IEEE}
}
@inproceedings{romero2018mage,
  title={Mage: Online and interference-aware scheduling for multi-scale heterogeneous systems},
  author={Romero and others},
  booktitle={PACT},
  pages={1--13},
  year={2018}
}
@inproceedings{delimitrou2013ibench,
  title={ibench: Quantifying interference for datacenter applications},
  author={Delimitrou and others},
  booktitle={IISWC},
  pages={23--33},
  year={2013},
  organization={IEEE}
}
@inproceedings{alves2020interference,
  title={An Interference-Aware Strategy for Co-locating High Performance Computing Applications in Clouds},
  author={Alves and others},
  booktitle={Symposium on High Performance Computing Systems},
  pages={3--20},
  year={2020},
  organization={Springer}
}
@inproceedings{patel2020clite,
  title={Clite: Efficient and qos-aware co-location of multiple latency-critical jobs for warehouse scale computers},
  author={Patel and others},
  booktitle={HPCA},
  pages={193--206},
  year={2020},
  organization={IEEE}
}
@inproceedings{alipourfard2017cherrypick,
  title={$\{$CherryPick$\}$: Adaptively Unearthing the Best Cloud Configurations for Big Data Analytics},
  author={Alipourfard and others},
  booktitle={14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
  pages={469--482},
  year={2017}
}
@ARTICLE{9747991,
  author={Rotem and others},
  journal={IEEE Micro}, 
  title={Intel Alder Lake CPU Architectures}, 
  year={2022},
  volume={42},
  number={3},
  pages={13-19},
  doi={10.1109/MM.2022.3164338}}

@inproceedings{lee2018pretzel,
  title={PRETZEL: Opening the Black Box of Machine Learning Prediction Serving Systems.},
  author={Lee and others},
  booktitle={OSDI},
  volume={18},
  pages={611--626},
  year={2018}
}


@inproceedings{zhang2019mark,
  title={MArk: Exploiting Cloud Services for Cost-Effective, SLO-Aware Machine Learning Inference Serving.},
  author={Zhang and others},
  booktitle={USENIX Annual Technical Conference},
  pages={1049--1062},
  year={2019}
}

@inproceedings{mendoza2021interference,
  title={Interference-aware scheduling for inference serving},
  author={Mendoza and others},
  booktitle={Proceedings of the 1st Workshop on Machine Learning and Systems},
  pages={80--88},
  year={2021}
}

@inproceedings{yeung2020horus,
  title={Horus: An interference-aware resource manager for deep learning systems},
  author={Yeung and others},
  booktitle={ICA3PP},
  pages={492--508},
  year={2020},
  organization={Springer}
}

@article{delimitrou2014quasar,
  title={Quasar: Resource-efficient and QoS-aware cluster management},
  author={Delimitrou, Christina and Kozyrakis, Christos},
  journal={ACM SIGPLAN Notices},
  volume={49},
  number={4},
  pages={127--144},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{chen2017prophet,
  title={Prophet: Precise qos prediction on non-preemptive accelerators to improve utilization in warehouse-scale computers},
  author={Chen, Quan and Yang, Hailong and Guo, Minyi and Kannan, Ram Srivatsa and Mars, Jason and Tang, Lingjia},
  booktitle={Proceedings of the 22nd ASPLOS'17},
  pages={17--32}
}

@article{chen2016baymax,
  title={Baymax: Qos awareness and increased utilization for non-preemptive accelerators in warehouse scale computers},
  author={Chen, Quan and Yang, Hailong and Mars, Jason and Tang, Lingjia},
  journal={ACM SIGPLAN Notices},
  volume={51},
  number={4},
  pages={681--696},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@inproceedings{lo2015heracles,
  title={Heracles: Improving resource efficiency at scale},
  author={Lo, David and Cheng, Liqun and Govindaraju, Rama and Ranganathan, Parthasarathy and Kozyrakis, Christos},
  booktitle={Proceedings of the 42nd Annual International Symposium on Computer Architecture},
  pages={450--462},
  year={2015}
}

@inproceedings{crankshaw2017clipper,
  title={Clipper: A Low-Latency Online Prediction Serving System.},
  author={Crankshaw, Daniel and Wang, Xin and Zhou, Giulio and Franklin, Michael J and Gonzalez, Joseph E and Stoica, Ion},
  booktitle={NSDI},
  year={2017}
}

@article{olston2017tensorflow,
  title={Tensorflow-serving: Flexible, high-performance ml serving},
  author={Olston, Christopher and Fiedel, Noah and Gorovoy, Kiril and Harmsen, Jeremiah and Lao, Li and Li, Fangwei and Rajashekhar, Vinu and Ramesh, Sukriti and Soyke, Jordan},
  journal={arXiv preprint arXiv:1712.06139},
  year={2017}
}

@inproceedings{liberty2020elastic,
  title={Elastic machine learning algorithms in amazon sagemaker},
  author={Liberty, Edo and Karnin, Zohar and Xiang, Bing and Rouesnel, Laurence and Coskun, Baris and Nallapati, Ramesh and Delgado, Julio and Sadoughi, Amir and Astashonok, Yury and Das, Piali and others},
  booktitle={SIGMOD},
  pages={731--737},
  year={2020}
}

@inproceedings{romero2021infaas,
  title={INFaaS: Automated Model-less Inference Serving.},
  author={Romero, Francisco and Li, Qian and Yadwadkar, Neeraja J and Kozyrakis, Christos},
  booktitle={USENIX Annual Technical Conference},
  pages={397--411},
  year={2021}
}

@inproceedings{lemay2020perseus,
  title={Perseus: Characterizing performance and cost of multi-tenant serving for cnn models},
  author={LeMay, Matthew and Li, Shijian and Guo, Tian},
  booktitle={IC2E},
  pages={66--72},
  year={2020},
  organization={IEEE}
}

@inproceedings{ke2022hercules,
  title={Hercules: Heterogeneity-aware inference serving for at-scale personalized recommendation},
  author={Ke, Liu and Gupta, Udit and Hempsteadis, Mark and Wu, Carole-Jean and Lee, Hsien-Hsin S and Zhang, Xuan},
  booktitle={HPCA},
  pages={141--144},
  year={2022},
  organization={IEEE}
}

@inproceedings{narayanan2019pipedream,
  title={PipeDream: Generalized pipeline parallelism for DNN training},
  author={Narayanan, Deepak and Harlap, Aaron and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil R and Ganger, Gregory R and Gibbons, Phillip B and Zaharia, Matei},
  booktitle={Proceedings of the 27th ACM Symposium on Operating Systems Principles},
  pages={1--15},
  year={2019}
}

@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{fan2021dapple,
  title={DAPPLE: A pipelined data parallel approach for training large models},
  author={Fan, Shiqing and Rong, Yi and Meng, Chen and Cao, Zongyan and Wang, Siyu and Zheng, Zhen and Wu, Chuan and Long, Guoping and Yang, Jun and Xia, Lixue and others},
  booktitle={Proceedings of the 26th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
  pages={431--445},
  year={2021}
}

@inproceedings{li2021chimera,
  title={Chimera: efficiently training large-scale neural networks with bidirectional pipelines},
  author={Li, Shigang and Hoefler, Torsten},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}

@article{wang2019high,
  title={High-throughput cnn inference on embedded arm big. little multicore processors},
  author={Wang and others},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={10},
  pages={2254--2267},
  year={2019},
  publisher={IEEE}
}

@article{kang2020scheduling,
  title={Scheduling of deep learning applications onto heterogeneous processors in an embedded device},
  author={Kang, Duseok and Oh, Jinwoo and Choi, Jongwoo and Yi, Youngmin and Ha, Soonhoi},
  journal={IEEE Access},
  volume={8},
  year={2020},
  publisher={IEEE}
}

@article{jeong2021deep,
  title={Deep learning inference parallelization on heterogeneous processors with tensorrt},
  author={Jeong, EunJin and Kim, Jangryul and Tan, Samnieng and Lee, Jaeseong and Ha, Soonhoi},
  journal={IEEE Embedded Systems Letters},
  volume={14},
  number={1},
  pages={15--18},
  year={2021},
  publisher={IEEE}
}
@inproceedings{soomro2022shisha,
  title={Shisha: Online scheduling of CNN pipelines on heterogeneous architectures},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={PPAM 2022}
}

@inproceedings{soomro2021online,
  title={An online guided tuning approach to run cnn pipelines on edge devices},
  author={Soomro, Pirah Noor and Abduljabbar, Mustafa and Castrillon, Jeronimo and Peric{\`a}s, Miquel},
  booktitle={CF'21}
}

@article{chang2022pipebert,
  title={PipeBERT: High-throughput BERT Inference for ARM Big. LITTLE Multi-core Processors},
  author={Chang, Hung-Yang and Mozafari, Seyyed Hasan and Chen, Cheng and Clark, James J and Meyer, Brett H and Gross, Warren J},
  journal={Journal of Signal Processing Systems},
  pages={1--18},
  year={2022},
  publisher={Springer}
}

@article{ben2019demystifying,
  title={Demystifying parallel and distributed deep learning: An in-depth concurrency analysis},
  author={Ben-Nun, Tal and Hoefler, Torsten},
  journal={ACM Computing Surveys (CSUR)},
  year={2019},
  publisher={ACM New York, NY, USA}
}

@article{lee2015fly,
  title={On-the-fly pipeline parallelism},
  author={Lee, I-Ting Angelina and Leiserson, Charles E and Schardl, Tao B and Zhang, Zhunping and Sukha, Jim},
  journal={ACM Transactions on Parallel Computing (TOPC)},
  volume={2},
  number={3},
  pages={1--42},
  year={2015},
  publisher={ACM New York, NY, USA}
}
@misc{chollet2015keras,
  title={Keras},
  author={Chollet, Fran\c{c}ois and others},
  year={2015},
  howpublished={\url{https://keras.io}},
}
@misc{gitlink,   
    title = {cnn-benchmarks},   
    url = {https://github.com/jcjohnson/cnn-benchmarks},   
    author = {Justin Johnson},   
    year = {2017},   
    note = {Accessed on March 2nd, 2023} 
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

==> shisha/experimental_setup.tex <==
\subsection{Experimental setup}
We simulate the inference serving system by generating a database of execution times of individual neural network layers.
For the purpose of generating database, we run neural network layers on Intel Alder Lake~\cite{9747991}.
Intel Alder Lake is combination of $8$ $2$xP-Cores as Performance cores and $8$ $2$xE-Cores as Efficient cores. 
We consider set of 8 P-cores as a single execution place of the inference serving system. 
We also measure the execution time of layers during interference by co-running iBench~\cite{delimitrou2013ibench} interference benchmark. The database thus contains execution time of each layer when run in isolation as well as in presence of interference. 
To imitate the effect of colocated application on shared resources
we incorporated interference by contending shared resources, such as memory and CPUs. Two benchmarks from iBench suit $memBW$ and $CPU$ are used for this purpose.
Table~\ref{tab:interference_scenarios} shows all combinations of interference we have considered for simulating interference in inference serving systems. Figure~\ref{fig:experimental_setup} shows execution times of a single VGG16 layer in all scenarios listed in ~\ref{tab:interference_scenarios}. We recorded the execution times for all the layers in all interference scenarios in the database. The database is later used by simulator to calculate execution times for pipeline stages. We consider layers executed one after another with in a pipeline stage so the execution time of a stage is calculated as sum of execution times of each layer with respect to the execution mode the stage is going through. 
For implementing neural networks we used Keras~\cite{chollet2015keras} framework and pinning utility to assign cores to main application and interfering application. Although the execution times are higher than practice, this is due to the fact that we are not using GPUs to run the network layers and it is already observed in practice~\cite{gitlink} that networks layers do not show higher performance on CPUs.

\begin{table}[]
\begin{tabular}{@{}ll@{}}
\toprule
Mode of execution & Core assignment on Alder Lake                                \\ \midrule
A                 & CNN:{[}0-7{]}                                                \\
B                 & CNN: {[}0-7{]}, IBench-MemBW: {[}0{]}                        \\
C                 & CNN: {[}0-7{]}, IBench-MemBW: {[}0-1{]}                      \\
D                 & CNN: {[}0-7{]}, IBench-MemBW: {[}0-3{]}                      \\
E                 & CNN: {[}0-7{]}, IBench-MemBW: {[}0-7{]}                      \\
F                 & CNN: {[}0-7{]}, IBench-CPU: {[}0{]}                          \\
G                 & CNN: {[}0-7{]}, IBench-CPU: {[}0-1{]}                        \\
H                 & CNN: {[}0-7{]}, IBench-CPU: {[}0-3{]}                        \\
I                 & CNN: {[}0-7{]}, IBench-CPU: {[}0-7{]}                        \\
J                 & CNN: {[}0-3{]}, IBench-MemBW: {[}4-7{]}                      \\
K                 & CNN: {[}0-3{]}, IBench-CPU: {[}4-7{]}                        \\
L                 & CNN: {[}0-3{]}, IBench-CPU: {[}4-7{]}, IBench-MemBW{[}4-7{]} \\
\bottomrule
\end{tabular}
\caption{Interference scenarios}
\label{tab:interference_scenarios}
\end{table}
\begin{figure}[!h]
\centering
\includegraphics[width=0.5\linewidth]{shisha/figs/experimental_setup.pdf}
\caption{Performance impact of different interference scenarios on a single VGG16 layer executed on 8xP-Cores of Alder Lake}\label{fig:experimental_setup}
\end{figure}
